When is Multicalibration Post-Processing Necessary?

Calibration is a well-studied property of predictors which guarantees meaningful uncertainty estimates. Multicalibration is a related notion -- originating in algorithmic fairness -- which requires predictors to be simultaneously calibrated over a potentially complex and overlapping collection of protected subpopulations (such as groups defined by ethnicity, race, or income). We conduct the first comprehensive study evaluating the usefulness of multicalibration post-processing across a broad set of tabular, image, and language datasets for models spanning from simple decision trees to 90 million parameter fine-tuned LLMs. Our findings can be summarized as follows: (1) models which are calibrated out of the box tend to be relatively multicalibrated without any additional post-processing; (2) multicalibration post-processing can help inherently uncalibrated models and large vision and language models; and (3) traditional calibration measures may sometimes provide multicalibration implicitly. More generally, we also distill many independent observations which may be useful for practical and effective applications of multicalibration post-processing in real-world contexts. We also release a python package implementing multicalibration algorithms, available via `pip install multicalibration'.

==> figures/alternate_groups/tables/ACSIncome_table.tex <==
\begin{tabular}{llllll}
\toprule
\textbf{{Model}} & \textbf{{ECE}} $\downarrow$ & \textbf{{Max ECE}} $\downarrow$ & \textbf{{smECE}} $\downarrow$ & \textbf{{Max smECE}} $\downarrow$ & \textbf{{Acc}} $\uparrow$ \\
\midrule
\rowcolor{Wheat1} MLP ERM & 0.014 ± 0.005 & 0.059 ± 0.007 & 0.015 ± 0.004 & 0.059 ± 0.008 & 0.811 ± 0.002 \\
\rowcolor{Wheat1} MLP $\hkrr$ & \highest{0.009 ± 0.003} & \highest{0.037 ± 0.005} & \highest{0.009 ± 0.003} & \highest{0.035 ± 0.003} & 0.803 ± 0.001 \\
\rowcolor{Wheat1} MLP $\hjz$ & 0.019 ± 0.003 & 0.053 ± 0.01 & 0.02 ± 0.002 & 0.051 ± 0.011 & 0.807 ± 0.004 \\
\rowcolor{Wheat1} MLP Platt & 0.012 ± 0.004 & 0.046 ± 0.008 & 0.014 ± 0.002 & 0.044 ± 0.007 & 0.811 ± 0.001 \\
\rowcolor{Wheat1} MLP Temp & 0.012 ± 0.005 & 0.056 ± 0.005 & 0.013 ± 0.004 & 0.056 ± 0.005 & 0.811 ± 0.001 \\
\rowcolor{Wheat1} MLP Isotonic & 0.012 ± 0.002 & 0.055 ± 0.005 & 0.013 ± 0.001 & 0.054 ± 0.006 & \highest{0.811 ± 0.001} \\
\midrule
RandomForest ERM & 0.01 ± 0.001 & 0.036 ± 0.001 & 0.011 ± 0.0 & 0.035 ± 0.001 & 0.819 ± 0.001 \\
RandomForest $\hkrr$ & 0.007 ± 0.001 & 0.043 ± 0.011 & \highest{0.007 ± 0.001} & 0.042 ± 0.01 & 0.818 ± 0.0 \\
RandomForest $\hjz$ & \highest{0.007 ± 0.001} & 0.032 ± 0.005 & 0.011 ± 0.001 & 0.031 ± 0.003 & 0.813 ± 0.007 \\
RandomForest Platt & 0.009 ± 0.001 & \highest{0.031 ± 0.003} & 0.011 ± 0.001 & \highest{0.029 ± 0.002} & 0.816 ± 0.004 \\
RandomForest Temp & 0.027 ± 0.001 & 0.074 ± 0.001 & 0.027 ± 0.001 & 0.073 ± 0.0 & \highest{0.819 ± 0.001} \\
RandomForest Isotonic & 0.008 ± 0.001 & 0.033 ± 0.001 & 0.011 ± 0.0 & 0.031 ± 0.001 & 0.818 ± 0.001 \\
\midrule
\rowcolor{Wheat1} SVM ERM & 0.216 ± 0.001 & 0.292 ± 0.004 & 0.109 ± 0.0 & 0.149 ± 0.002 & \highest{0.784 ± 0.001} \\
\rowcolor{Wheat1} SVM $\hkrr$ & \highest{0.008 ± 0.0} & \highest{0.034 ± 0.005} & \highest{0.008 ± 0.0} & \highest{0.032 ± 0.004} & 0.667 ± 0.0 \\
\rowcolor{Wheat1} SVM $\hjz$ & 0.013 ± 0.002 & 0.164 ± 0.009 & 0.019 ± 0.001 & 0.163 ± 0.009 & 0.665 ± 0.0 \\
\rowcolor{Wheat1} SVM Platt & 0.336 ± 0.007 & 0.438 ± 0.0 & 0.168 ± 0.004 & 0.214 ± 0.0 & 0.664 ± 0.007 \\
\rowcolor{Wheat1} SVM Temp & 0.099 ± 0.006 & 0.216 ± 0.0 & 0.099 ± 0.006 & 0.211 ± 0.0 & 0.678 ± 0.006 \\
\rowcolor{Wheat1} SVM Isotonic & 0.081 ± 0.012 & 0.263 ± 0.014 & 0.081 ± 0.012 & 0.25 ± 0.011 & 0.664 ± 0.007 \\
\midrule
LogisticRegression ERM & 0.012 ± 0.002 & 0.123 ± 0.014 & 0.015 ± 0.002 & 0.116 ± 0.012 & 0.779 ± 0.007 \\
LogisticRegression $\hkrr$ & 0.006 ± 0.002 & \highest{0.041 ± 0.003} & \highest{0.006 ± 0.002} & \highest{0.038 ± 0.002} & \highest{0.78 ± 0.007} \\
LogisticRegression $\hjz$ & 0.011 ± 0.001 & 0.085 ± 0.013 & 0.014 ± 0.001 & 0.083 ± 0.012 & 0.775 ± 0.009 \\
LogisticRegression Platt & 0.021 ± 0.004 & 0.108 ± 0.017 & 0.021 ± 0.004 & 0.105 ± 0.015 & 0.774 ± 0.012 \\
LogisticRegression Temp & 0.019 ± 0.0 & 0.115 ± 0.004 & 0.02 ± 0.0 & 0.111 ± 0.005 & 0.776 ± 0.009 \\
LogisticRegression Isotonic & \highest{0.005 ± 0.001} & 0.109 ± 0.007 & 0.009 ± 0.001 & 0.105 ± 0.004 & 0.775 ± 0.009 \\
\midrule
\rowcolor{Wheat1} DecisionTree ERM & 0.017 ± 0.001 & 0.051 ± 0.004 & 0.016 ± 0.001 & 0.048 ± 0.004 & \highest{0.804 ± 0.0} \\
\rowcolor{Wheat1} DecisionTree $\hkrr$ & 0.008 ± 0.001 & 0.041 ± 0.004 & \highest{0.008 ± 0.001} & 0.039 ± 0.003 & 0.799 ± 0.001 \\
\rowcolor{Wheat1} DecisionTree $\hjz$ & 0.019 ± 0.001 & 0.049 ± 0.002 & 0.017 ± 0.002 & 0.046 ± 0.002 & 0.802 ± 0.001 \\
\rowcolor{Wheat1} DecisionTree Platt & 0.011 ± 0.001 & \highest{0.041 ± 0.006} & 0.013 ± 0.001 & \highest{0.037 ± 0.005} & 0.803 ± 0.0 \\
\rowcolor{Wheat1} DecisionTree Temp & 0.028 ± 0.002 & 0.073 ± 0.001 & 0.027 ± 0.002 & 0.072 ± 0.001 & 0.803 ± 0.001 \\
\rowcolor{Wheat1} DecisionTree Isotonic & \highest{0.007 ± 0.002} & 0.054 ± 0.003 & 0.01 ± 0.001 & 0.051 ± 0.003 & 0.803 ± 0.001 \\
\midrule
NaiveBayes ERM & 0.117 ± 0.0 & 0.201 ± 0.001 & 0.109 ± 0.0 & 0.182 ± 0.0 & 0.754 ± 0.0 \\
NaiveBayes $\hkrr$ & \highest{0.006 ± 0.001} & \highest{0.042 ± 0.005} & \highest{0.006 ± 0.001} & \highest{0.039 ± 0.004} & \highest{0.77 ± 0.001} \\
NaiveBayes $\hjz$ & 0.017 ± 0.002 & 0.093 ± 0.006 & 0.021 ± 0.001 & 0.091 ± 0.007 & 0.762 ± 0.004 \\
NaiveBayes Platt & 0.085 ± 0.004 & 0.165 ± 0.007 & 0.08 ± 0.004 & 0.161 ± 0.006 & 0.756 ± 0.002 \\
NaiveBayes Temp & 0.079 ± 0.002 & 0.182 ± 0.002 & 0.069 ± 0.001 & 0.18 ± 0.002 & 0.754 ± 0.001 \\
NaiveBayes Isotonic & 0.008 ± 0.002 & 0.105 ± 0.001 & 0.011 ± 0.002 & 0.103 ± 0.001 & 0.768 ± 0.0 \\
\bottomrule
\end{tabular}


==> figures/alternate_groups/tables/BankMarketing_table.tex <==
\begin{tabular}{llllll}
\toprule
\textbf{{Model}} & \textbf{{ECE}} $\downarrow$ & \textbf{{Max ECE}} $\downarrow$ & \textbf{{smECE}} $\downarrow$ & \textbf{{Max smECE}} $\downarrow$ & \textbf{{Acc}} $\uparrow$ \\
\midrule
\rowcolor{Wheat1} MLP ERM & 0.008 ± 0.003 & 0.14 ± 0.018 & 0.012 ± 0.002 & 0.099 ± 0.009 & 0.9 ± 0.001 \\
\rowcolor{Wheat1} MLP $\hkrr$ & 0.102 ± 0.003 & 0.127 ± 0.013 & 0.098 ± 0.001 & 0.117 ± 0.016 & 0.879 ± 0.0 \\
\rowcolor{Wheat1} MLP $\hjz$ & 0.019 ± 0.012 & 0.137 ± 0.016 & 0.021 ± 0.011 & 0.09 ± 0.008 & \highest{0.901 ± 0.001} \\
\rowcolor{Wheat1} MLP Platt & 0.011 ± 0.004 & 0.138 ± 0.022 & 0.014 ± 0.003 & 0.105 ± 0.017 & 0.896 ± 0.005 \\
\rowcolor{Wheat1} MLP Temp & 0.042 ± 0.01 & \highest{0.123 ± 0.024} & 0.042 ± 0.01 & \highest{0.074 ± 0.007} & 0.901 ± 0.001 \\
\rowcolor{Wheat1} MLP Isotonic & \highest{0.008 ± 0.002} & 0.126 ± 0.024 & \highest{0.01 ± 0.001} & 0.091 ± 0.009 & 0.9 ± 0.001 \\
\midrule
RandomForest ERM & 0.014 ± 0.001 & 0.095 ± 0.01 & 0.015 ± 0.0 & 0.062 ± 0.001 & 0.903 ± 0.002 \\
RandomForest $\hkrr$ & 0.012 ± 0.002 & 0.106 ± 0.017 & 0.012 ± 0.002 & 0.082 ± 0.008 & 0.898 ± 0.001 \\
RandomForest $\hjz$ & 0.011 ± 0.003 & 0.108 ± 0.022 & 0.013 ± 0.002 & 0.066 ± 0.014 & \highest{0.903 ± 0.001} \\
RandomForest Platt & 0.009 ± 0.002 & \highest{0.095 ± 0.022} & 0.012 ± 0.001 & \highest{0.06 ± 0.006} & 0.903 ± 0.001 \\
RandomForest Temp & 0.057 ± 0.001 & 0.117 ± 0.019 & 0.054 ± 0.001 & 0.083 ± 0.002 & 0.903 ± 0.001 \\
RandomForest Isotonic & \highest{0.008 ± 0.002} & 0.116 ± 0.024 & \highest{0.011 ± 0.001} & 0.083 ± 0.009 & 0.901 ± 0.001 \\
\midrule
\rowcolor{Wheat1} SVM ERM & 0.106 ± 0.001 & 0.347 ± 0.027 & 0.053 ± 0.001 & 0.173 ± 0.013 & \highest{0.894 ± 0.001} \\
\rowcolor{Wheat1} SVM $\hkrr$ & 0.051 ± 0.014 & \highest{0.108 ± 0.038} & 0.051 ± 0.014 & \highest{0.091 ± 0.028} & 0.879 ± 0.0 \\
\rowcolor{Wheat1} SVM $\hjz$ & 0.106 ± 0.001 & 0.134 ± 0.003 & 0.098 ± 0.0 & 0.112 ± 0.004 & 0.879 ± 0.0 \\
\rowcolor{Wheat1} SVM Platt & 0.117 ± 0.001 & 0.36 ± 0.009 & 0.059 ± 0.001 & 0.178 ± 0.004 & 0.883 ± 0.001 \\
\rowcolor{Wheat1} SVM Temp & 0.152 ± 0.003 & 0.225 ± 0.0 & 0.151 ± 0.003 & 0.219 ± 0.0 & 0.88 ± 0.001 \\
\rowcolor{Wheat1} SVM Isotonic & \highest{0.023 ± 0.009} & 0.247 ± 0.025 & \highest{0.023 ± 0.009} & 0.237 ± 0.021 & 0.88 ± 0.001 \\
\midrule
LogisticRegression ERM & 0.032 ± 0.001 & 0.154 ± 0.006 & 0.03 ± 0.001 & 0.12 ± 0.002 & 0.899 ± 0.001 \\
LogisticRegression $\hkrr$ & 0.018 ± 0.002 & 0.132 ± 0.027 & 0.018 ± 0.002 & 0.108 ± 0.027 & 0.897 ± 0.002 \\
LogisticRegression $\hjz$ & 0.106 ± 0.001 & 0.134 ± 0.003 & 0.098 ± 0.0 & 0.112 ± 0.004 & 0.879 ± 0.0 \\
LogisticRegression Platt & 0.023 ± 0.005 & 0.156 ± 0.009 & 0.023 ± 0.004 & 0.129 ± 0.012 & 0.897 ± 0.002 \\
LogisticRegression Temp & 0.061 ± 0.001 & 0.174 ± 0.02 & 0.056 ± 0.0 & 0.121 ± 0.005 & 0.899 ± 0.001 \\
LogisticRegression Isotonic & \highest{0.008 ± 0.001} & \highest{0.114 ± 0.012} & \highest{0.011 ± 0.002} & \highest{0.093 ± 0.006} & \highest{0.9 ± 0.001} \\
\midrule
\rowcolor{Wheat1} DecisionTree ERM & 0.028 ± 0.002 & 0.213 ± 0.021 & 0.022 ± 0.001 & 0.154 ± 0.016 & \highest{0.897 ± 0.002} \\
\rowcolor{Wheat1} DecisionTree $\hkrr$ & 0.102 ± 0.003 & \highest{0.127 ± 0.013} & 0.098 ± 0.001 & 0.117 ± 0.016 & 0.879 ± 0.0 \\
\rowcolor{Wheat1} DecisionTree $\hjz$ & 0.106 ± 0.001 & 0.134 ± 0.003 & 0.098 ± 0.0 & \highest{0.112 ± 0.004} & 0.879 ± 0.0 \\
\rowcolor{Wheat1} DecisionTree Platt & 0.025 ± 0.006 & 0.214 ± 0.044 & 0.021 ± 0.002 & 0.153 ± 0.019 & 0.897 ± 0.002 \\
\rowcolor{Wheat1} DecisionTree Temp & 0.116 ± 0.001 & 0.173 ± 0.013 & 0.114 ± 0.001 & 0.163 ± 0.003 & 0.896 ± 0.002 \\
\rowcolor{Wheat1} DecisionTree Isotonic & \highest{0.01 ± 0.002} & 0.157 ± 0.011 & \highest{0.011 ± 0.002} & 0.139 ± 0.014 & 0.896 ± 0.002 \\
\midrule
NaiveBayes ERM & 0.122 ± 0.003 & 0.521 ± 0.002 & 0.093 ± 0.002 & 0.308 ± 0.002 & 0.857 ± 0.003 \\
NaiveBayes $\hkrr$ & 0.037 ± 0.005 & 0.121 ± 0.024 & 0.036 ± 0.004 & 0.106 ± 0.016 & 0.872 ± 0.003 \\
NaiveBayes $\hjz$ & 0.106 ± 0.001 & 0.134 ± 0.003 & 0.098 ± 0.0 & 0.112 ± 0.004 & 0.879 ± 0.0 \\
NaiveBayes Platt & 0.122 ± 0.005 & 0.528 ± 0.01 & 0.094 ± 0.004 & 0.318 ± 0.012 & 0.857 ± 0.004 \\
NaiveBayes Temp & 0.217 ± 0.002 & 0.293 ± 0.009 & 0.212 ± 0.002 & 0.268 ± 0.009 & 0.857 ± 0.004 \\
NaiveBayes Isotonic & \highest{0.007 ± 0.001} & \highest{0.118 ± 0.011} & \highest{0.01 ± 0.001} & \highest{0.095 ± 0.012} & \highest{0.885 ± 0.002} \\
\bottomrule
\end{tabular}


==> figures/alternate_groups/tables/CreditDefault_table.tex <==
\begin{tabular}{llllll}
\toprule
\textbf{{Model}} & \textbf{{ECE}} $\downarrow$ & \textbf{{Max ECE}} $\downarrow$ & \textbf{{smECE}} $\downarrow$ & \textbf{{Max smECE}} $\downarrow$ & \textbf{{Acc}} $\uparrow$ \\
\midrule
\rowcolor{Wheat1} MLP ERM & 0.018 ± 0.005 & 0.039 ± 0.004 & 0.019 ± 0.004 & 0.035 ± 0.003 & 0.818 ± 0.001 \\
\rowcolor{Wheat1} MLP $\hkrr$ & 0.028 ± 0.003 & \highest{0.026 ± 0.003} & 0.026 ± 0.002 & \highest{0.025 ± 0.002} & 0.781 ± 0.0 \\
\rowcolor{Wheat1} MLP $\hjz$ & 0.033 ± 0.002 & 0.036 ± 0.008 & 0.03 ± 0.001 & 0.028 ± 0.002 & 0.781 ± 0.0 \\
\rowcolor{Wheat1} MLP Platt & 0.013 ± 0.004 & 0.043 ± 0.008 & 0.015 ± 0.002 & 0.038 ± 0.008 & \highest{0.82 ± 0.0} \\
\rowcolor{Wheat1} MLP Temp & 0.016 ± 0.004 & 0.043 ± 0.007 & 0.018 ± 0.003 & 0.033 ± 0.002 & 0.819 ± 0.001 \\
\rowcolor{Wheat1} MLP Isotonic & \highest{0.011 ± 0.003} & 0.043 ± 0.005 & \highest{0.014 ± 0.001} & 0.035 ± 0.004 & 0.818 ± 0.001 \\
\midrule
RandomForest ERM & 0.019 ± 0.001 & 0.035 ± 0.003 & 0.02 ± 0.001 & 0.033 ± 0.001 & \highest{0.82 ± 0.001} \\
RandomForest $\hkrr$ & 0.028 ± 0.003 & \highest{0.026 ± 0.003} & 0.026 ± 0.002 & \highest{0.025 ± 0.002} & 0.781 ± 0.0 \\
RandomForest $\hjz$ & 0.033 ± 0.002 & 0.036 ± 0.008 & 0.03 ± 0.001 & 0.028 ± 0.002 & 0.781 ± 0.0 \\
RandomForest Platt & \highest{0.013 ± 0.002} & 0.04 ± 0.007 & 0.016 ± 0.002 & 0.035 ± 0.003 & 0.819 ± 0.001 \\
RandomForest Temp & 0.023 ± 0.003 & 0.04 ± 0.003 & 0.024 ± 0.002 & 0.037 ± 0.003 & 0.819 ± 0.001 \\
RandomForest Isotonic & 0.013 ± 0.003 & 0.035 ± 0.002 & \highest{0.015 ± 0.002} & 0.031 ± 0.002 & 0.819 ± 0.001 \\
\midrule
\rowcolor{Wheat1} SVM ERM & 0.181 ± 0.0 & 0.21 ± 0.001 & 0.091 ± 0.0 & 0.105 ± 0.0 & 0.819 ± 0.0 \\
\rowcolor{Wheat1} SVM $\hkrr$ & 0.02 ± 0.001 & 0.046 ± 0.004 & 0.016 ± 0.001 & 0.031 ± 0.003 & 0.819 ± 0.001 \\
\rowcolor{Wheat1} SVM $\hjz$ & 0.033 ± 0.002 & 0.036 ± 0.008 & 0.03 ± 0.001 & 0.028 ± 0.002 & 0.781 ± 0.0 \\
\rowcolor{Wheat1} SVM Platt & 0.18 ± 0.001 & 0.213 ± 0.002 & 0.09 ± 0.0 & 0.106 ± 0.001 & \highest{0.82 ± 0.001} \\
\rowcolor{Wheat1} SVM Temp & 0.022 ± 0.0 & 0.052 ± 0.001 & 0.022 ± 0.0 & 0.051 ± 0.001 & 0.82 ± 0.0 \\
\rowcolor{Wheat1} SVM Isotonic & \highest{0.006 ± 0.001} & \highest{0.026 ± 0.002} & \highest{0.006 ± 0.001} & \highest{0.026 ± 0.002} & \highest{0.82 ± 0.001} \\
\midrule
LogisticRegression ERM & \highest{0.01 ± 0.001} & 0.042 ± 0.004 & 0.015 ± 0.001 & 0.036 ± 0.003 & 0.819 ± 0.0 \\
LogisticRegression $\hkrr$ & 0.028 ± 0.003 & \highest{0.026 ± 0.003} & 0.026 ± 0.002 & \highest{0.025 ± 0.002} & 0.781 ± 0.0 \\
LogisticRegression $\hjz$ & 0.033 ± 0.002 & 0.036 ± 0.008 & 0.03 ± 0.001 & 0.028 ± 0.002 & 0.781 ± 0.0 \\
LogisticRegression Platt & 0.014 ± 0.001 & 0.045 ± 0.004 & 0.016 ± 0.002 & 0.037 ± 0.003 & 0.819 ± 0.0 \\
LogisticRegression Temp & 0.023 ± 0.001 & 0.041 ± 0.006 & 0.023 ± 0.001 & 0.037 ± 0.001 & 0.819 ± 0.0 \\
LogisticRegression Isotonic & 0.01 ± 0.002 & 0.04 ± 0.009 & \highest{0.014 ± 0.001} & 0.034 ± 0.006 & \highest{0.82 ± 0.001} \\
\midrule
\rowcolor{Wheat1} DecisionTree ERM & 0.04 ± 0.003 & 0.078 ± 0.011 & 0.031 ± 0.001 & 0.054 ± 0.006 & 0.81 ± 0.003 \\
\rowcolor{Wheat1} DecisionTree $\hkrr$ & 0.028 ± 0.003 & \highest{0.026 ± 0.003} & 0.026 ± 0.002 & \highest{0.025 ± 0.002} & 0.781 ± 0.0 \\
\rowcolor{Wheat1} DecisionTree $\hjz$ & 0.033 ± 0.002 & 0.036 ± 0.008 & 0.03 ± 0.001 & 0.028 ± 0.002 & 0.781 ± 0.0 \\
\rowcolor{Wheat1} DecisionTree Platt & 0.033 ± 0.003 & 0.062 ± 0.005 & 0.028 ± 0.002 & 0.05 ± 0.006 & 0.81 ± 0.003 \\
\rowcolor{Wheat1} DecisionTree Temp & 0.031 ± 0.004 & 0.062 ± 0.009 & 0.029 ± 0.003 & 0.058 ± 0.01 & \highest{0.811 ± 0.003} \\
\rowcolor{Wheat1} DecisionTree Isotonic & \highest{0.007 ± 0.001} & 0.04 ± 0.006 & \highest{0.009 ± 0.003} & 0.036 ± 0.007 & 0.797 ± 0.004 \\
\midrule
NaiveBayes ERM & 0.187 ± 0.006 & 0.226 ± 0.005 & 0.108 ± 0.005 & 0.132 ± 0.007 & 0.807 ± 0.004 \\
NaiveBayes $\hkrr$ & 0.028 ± 0.013 & \highest{0.035 ± 0.008} & 0.026 ± 0.013 & 0.03 ± 0.006 & 0.784 ± 0.02 \\
NaiveBayes $\hjz$ & 0.033 ± 0.002 & 0.036 ± 0.008 & 0.03 ± 0.001 & \highest{0.028 ± 0.002} & 0.781 ± 0.0 \\
NaiveBayes Platt & 0.197 ± 0.011 & 0.236 ± 0.013 & 0.119 ± 0.015 & 0.143 ± 0.023 & 0.792 ± 0.014 \\
NaiveBayes Temp & 0.037 ± 0.012 & 0.075 ± 0.007 & 0.037 ± 0.012 & 0.073 ± 0.008 & 0.809 ± 0.003 \\
NaiveBayes Isotonic & \highest{0.013 ± 0.004} & 0.039 ± 0.007 & \highest{0.016 ± 0.003} & 0.037 ± 0.005 & \highest{0.809 ± 0.001} \\
\bottomrule
\end{tabular}


==> figures/alternate_groups/tables/HMDA_table.tex <==
\begin{tabular}{llllll}
\toprule
\textbf{{Model}} & \textbf{{ECE}} $\downarrow$ & \textbf{{Max ECE}} $\downarrow$ & \textbf{{smECE}} $\downarrow$ & \textbf{{Max smECE}} $\downarrow$ & \textbf{{Acc}} $\uparrow$ \\
\midrule
\rowcolor{Wheat1} MLP ERM & 0.045 ± 0.015 & 0.087 ± 0.018 & 0.043 ± 0.014 & 0.084 ± 0.018 & 0.834 ± 0.002 \\
\rowcolor{Wheat1} MLP $\hkrr$ & \highest{0.004 ± 0.001} & \highest{0.034 ± 0.006} & \highest{0.004 ± 0.001} & \highest{0.033 ± 0.006} & 0.756 ± 0.0 \\
\rowcolor{Wheat1} MLP $\hjz$ & 0.012 ± 0.001 & 0.062 ± 0.021 & 0.016 ± 0.001 & 0.056 ± 0.019 & \highest{0.835 ± 0.009} \\
\rowcolor{Wheat1} MLP Platt & 0.184 ± 0.009 & 0.272 ± 0.025 & 0.14 ± 0.002 & 0.206 ± 0.017 & 0.781 ± 0.002 \\
\rowcolor{Wheat1} MLP Temp & 0.047 ± 0.033 & 0.097 ± 0.02 & 0.046 ± 0.032 & 0.094 ± 0.02 & 0.817 ± 0.008 \\
\rowcolor{Wheat1} MLP Isotonic & 0.013 ± 0.002 & 0.1 ± 0.009 & 0.014 ± 0.002 & 0.092 ± 0.008 & 0.824 ± 0.006 \\
\midrule
RandomForest ERM & 0.038 ± 0.002 & 0.054 ± 0.001 & 0.038 ± 0.002 & 0.053 ± 0.001 & 0.868 ± 0.001 \\
RandomForest $\hkrr$ & \highest{0.006 ± 0.001} & \highest{0.028 ± 0.003} & \highest{0.006 ± 0.001} & \highest{0.027 ± 0.003} & 0.866 ± 0.001 \\
RandomForest $\hjz$ & 0.007 ± 0.002 & 0.044 ± 0.008 & 0.011 ± 0.002 & 0.041 ± 0.007 & 0.869 ± 0.001 \\
RandomForest Platt & 0.009 ± 0.001 & 0.06 ± 0.007 & 0.011 ± 0.001 & 0.054 ± 0.005 & 0.867 ± 0.001 \\
RandomForest Temp & 0.037 ± 0.001 & 0.072 ± 0.004 & 0.039 ± 0.001 & 0.07 ± 0.004 & 0.866 ± 0.001 \\
RandomForest Isotonic & 0.009 ± 0.002 & 0.048 ± 0.002 & 0.01 ± 0.002 & 0.046 ± 0.003 & \highest{0.869 ± 0.001} \\
\midrule
\rowcolor{Wheat1} SVM ERM & 0.144 ± 0.001 & 0.31 ± 0.004 & 0.072 ± 0.0 & 0.158 ± 0.002 & \highest{0.856 ± 0.001} \\
\rowcolor{Wheat1} SVM $\hkrr$ & 0.004 ± 0.001 & \highest{0.034 ± 0.006} & 0.004 ± 0.001 & \highest{0.033 ± 0.006} & 0.756 ± 0.0 \\
\rowcolor{Wheat1} SVM $\hjz$ & 0.008 ± 0.002 & 0.058 ± 0.009 & 0.011 ± 0.001 & 0.058 ± 0.009 & 0.754 ± 0.0 \\
\rowcolor{Wheat1} SVM Platt & 0.008 ± 0.002 & 0.079 ± 0.002 & 0.012 ± 0.001 & 0.079 ± 0.001 & 0.754 ± 0.0 \\
\rowcolor{Wheat1} SVM Temp & 0.266 ± 0.001 & 0.324 ± 0.005 & 0.253 ± 0.001 & 0.295 ± 0.003 & 0.647 ± 0.003 \\
\rowcolor{Wheat1} SVM Isotonic & \highest{0.002 ± 0.001} & 0.115 ± 0.001 & \highest{0.002 ± 0.001} & 0.115 ± 0.001 & 0.754 ± 0.0 \\
\midrule
LogisticRegression ERM & 0.016 ± 0.001 & 0.171 ± 0.002 & 0.016 ± 0.001 & 0.168 ± 0.002 & 0.827 ± 0.001 \\
LogisticRegression $\hkrr$ & 0.007 ± 0.002 & \highest{0.028 ± 0.005} & 0.007 ± 0.002 & \highest{0.026 ± 0.005} & \highest{0.862 ± 0.0} \\
LogisticRegression $\hjz$ & 0.006 ± 0.002 & 0.039 ± 0.007 & 0.011 ± 0.002 & 0.037 ± 0.006 & 0.857 ± 0.003 \\
LogisticRegression Platt & 0.008 ± 0.002 & 0.079 ± 0.002 & 0.012 ± 0.001 & 0.079 ± 0.001 & 0.754 ± 0.0 \\
LogisticRegression Temp & 0.062 ± 0.006 & 0.17 ± 0.039 & 0.058 ± 0.005 & 0.166 ± 0.042 & 0.833 ± 0.011 \\
LogisticRegression Isotonic & \highest{0.002 ± 0.001} & 0.115 ± 0.001 & \highest{0.002 ± 0.001} & 0.115 ± 0.001 & 0.754 ± 0.0 \\
\midrule
\rowcolor{Wheat1} DecisionTree ERM & 0.019 ± 0.001 & 0.039 ± 0.005 & 0.018 ± 0.002 & 0.038 ± 0.003 & 0.863 ± 0.001 \\
\rowcolor{Wheat1} DecisionTree $\hkrr$ & \highest{0.005 ± 0.001} & \highest{0.033 ± 0.008} & \highest{0.005 ± 0.001} & 0.032 ± 0.007 & 0.856 ± 0.001 \\
\rowcolor{Wheat1} DecisionTree $\hjz$ & 0.016 ± 0.003 & 0.042 ± 0.004 & 0.015 ± 0.002 & 0.036 ± 0.003 & 0.862 ± 0.0 \\
\rowcolor{Wheat1} DecisionTree Platt & 0.02 ± 0.002 & 0.051 ± 0.007 & 0.018 ± 0.002 & 0.046 ± 0.007 & 0.861 ± 0.001 \\
\rowcolor{Wheat1} DecisionTree Temp & 0.06 ± 0.002 & 0.08 ± 0.002 & 0.052 ± 0.001 & 0.069 ± 0.003 & 0.863 ± 0.002 \\
\rowcolor{Wheat1} DecisionTree Isotonic & 0.006 ± 0.001 & 0.034 ± 0.004 & 0.009 ± 0.002 & \highest{0.032 ± 0.003} & \highest{0.863 ± 0.001} \\
\midrule
NaiveBayes ERM & 0.134 ± 0.001 & 0.416 ± 0.006 & 0.126 ± 0.0 & 0.324 ± 0.003 & 0.808 ± 0.001 \\
NaiveBayes $\hkrr$ & 0.006 ± 0.001 & \highest{0.032 ± 0.005} & 0.006 ± 0.001 & \highest{0.03 ± 0.003} & \highest{0.848 ± 0.001} \\
NaiveBayes $\hjz$ & 0.008 ± 0.002 & 0.058 ± 0.009 & 0.011 ± 0.001 & 0.058 ± 0.009 & 0.754 ± 0.0 \\
NaiveBayes Platt & 0.008 ± 0.002 & 0.079 ± 0.002 & 0.012 ± 0.001 & 0.079 ± 0.001 & 0.754 ± 0.0 \\
NaiveBayes Temp & 0.185 ± 0.002 & 0.271 ± 0.004 & 0.184 ± 0.002 & 0.257 ± 0.003 & 0.809 ± 0.0 \\
NaiveBayes Isotonic & \highest{0.002 ± 0.001} & 0.115 ± 0.001 & \highest{0.002 ± 0.001} & 0.115 ± 0.001 & 0.754 ± 0.0 \\
\bottomrule
\end{tabular}


==> figures/alternate_groups/tables/MEPS_table.tex <==
\begin{tabular}{llllll}
\toprule
\textbf{{Model}} & \textbf{{ECE}} $\downarrow$ & \textbf{{Max ECE}} $\downarrow$ & \textbf{{smECE}} $\downarrow$ & \textbf{{Max smECE}} $\downarrow$ & \textbf{{Acc}} $\uparrow$ \\
\midrule
\rowcolor{Wheat1} MLP ERM & \highest{0.017 ± 0.005} & 0.3 ± 0.057 & 0.021 ± 0.004 & 0.204 ± 0.03 & \highest{0.866 ± 0.002} \\
\rowcolor{Wheat1} MLP $\hkrr$ & 0.019 ± 0.002 & 0.311 ± 0.08 & \highest{0.018 ± 0.002} & 0.217 ± 0.043 & 0.84 ± 0.002 \\
\rowcolor{Wheat1} MLP $\hjz$ & 0.025 ± 0.006 & \highest{0.28 ± 0.049} & 0.024 ± 0.003 & 0.208 ± 0.031 & 0.864 ± 0.003 \\
\rowcolor{Wheat1} MLP Platt & 0.02 ± 0.004 & 0.314 ± 0.048 & 0.023 ± 0.002 & 0.239 ± 0.039 & 0.863 ± 0.002 \\
\rowcolor{Wheat1} MLP Temp & 0.063 ± 0.037 & 0.282 ± 0.061 & 0.058 ± 0.032 & \highest{0.195 ± 0.038} & 0.864 ± 0.003 \\
\rowcolor{Wheat1} MLP Isotonic & 0.025 ± 0.004 & 0.29 ± 0.047 & 0.025 ± 0.004 & 0.234 ± 0.027 & 0.864 ± 0.003 \\
\midrule
RandomForest ERM & 0.019 ± 0.001 & 0.297 ± 0.038 & 0.021 ± 0.001 & 0.228 ± 0.018 & \highest{0.863 ± 0.003} \\
RandomForest $\hkrr$ & 0.019 ± 0.002 & 0.311 ± 0.08 & 0.018 ± 0.002 & 0.217 ± 0.043 & 0.84 ± 0.002 \\
RandomForest $\hjz$ & 0.016 ± 0.002 & \highest{0.239 ± 0.036} & 0.019 ± 0.001 & \highest{0.211 ± 0.015} & 0.861 ± 0.002 \\
RandomForest Platt & 0.019 ± 0.005 & 0.267 ± 0.03 & 0.021 ± 0.001 & 0.229 ± 0.02 & 0.86 ± 0.003 \\
RandomForest Temp & 0.041 ± 0.004 & 0.283 ± 0.057 & 0.039 ± 0.004 & 0.236 ± 0.014 & 0.861 ± 0.002 \\
RandomForest Isotonic & \highest{0.015 ± 0.002} & 0.248 ± 0.019 & \highest{0.017 ± 0.001} & 0.235 ± 0.012 & 0.862 ± 0.002 \\
\midrule
\rowcolor{Wheat1} SVM ERM & 0.143 ± 0.002 & 0.565 ± 0.0 & 0.072 ± 0.001 & 0.265 ± 0.0 & 0.857 ± 0.002 \\
\rowcolor{Wheat1} SVM $\hkrr$ & \highest{0.019 ± 0.002} & \highest{0.311 ± 0.08} & \highest{0.018 ± 0.002} & \highest{0.217 ± 0.043} & 0.84 ± 0.002 \\
\rowcolor{Wheat1} SVM $\hjz$ & 0.027 ± 0.005 & 0.311 ± 0.037 & 0.026 ± 0.002 & 0.284 ± 0.027 & 0.826 ± 0.0 \\
\rowcolor{Wheat1} SVM Platt & 0.14 ± 0.001 & 0.47 ± 0.051 & 0.07 ± 0.001 & 0.229 ± 0.02 & \highest{0.86 ± 0.001} \\
\rowcolor{Wheat1} SVM Temp & 0.117 ± 0.011 & 0.323 ± 0.022 & 0.116 ± 0.011 & 0.277 ± 0.018 & 0.847 ± 0.01 \\
\rowcolor{Wheat1} SVM Isotonic & 0.048 ± 0.023 & 0.317 ± 0.076 & 0.048 ± 0.023 & 0.275 ± 0.052 & 0.847 ± 0.017 \\
\midrule
LogisticRegression ERM & 0.022 ± 0.002 & 0.26 ± 0.02 & 0.022 ± 0.001 & 0.184 ± 0.009 & \highest{0.866 ± 0.002} \\
LogisticRegression $\hkrr$ & 0.019 ± 0.002 & 0.311 ± 0.08 & \highest{0.018 ± 0.002} & 0.217 ± 0.043 & 0.84 ± 0.002 \\
LogisticRegression $\hjz$ & 0.017 ± 0.003 & 0.256 ± 0.064 & 0.02 ± 0.001 & 0.177 ± 0.028 & 0.863 ± 0.003 \\
LogisticRegression Platt & 0.02 ± 0.001 & 0.254 ± 0.032 & 0.022 ± 0.0 & 0.176 ± 0.031 & 0.862 ± 0.004 \\
LogisticRegression Temp & 0.102 ± 0.002 & \highest{0.207 ± 0.045} & 0.094 ± 0.001 & \highest{0.159 ± 0.025} & 0.862 ± 0.003 \\
LogisticRegression Isotonic & \highest{0.016 ± 0.002} & 0.233 ± 0.03 & 0.019 ± 0.002 & 0.188 ± 0.037 & 0.861 ± 0.005 \\
\midrule
\rowcolor{Wheat1} DecisionTree ERM & 0.067 ± 0.004 & 0.328 ± 0.036 & 0.047 ± 0.004 & \highest{0.189 ± 0.01} & \highest{0.85 ± 0.006} \\
\rowcolor{Wheat1} DecisionTree $\hkrr$ & \highest{0.019 ± 0.002} & 0.311 ± 0.08 & \highest{0.018 ± 0.002} & 0.217 ± 0.043 & 0.84 ± 0.002 \\
\rowcolor{Wheat1} DecisionTree $\hjz$ & 0.03 ± 0.007 & \highest{0.286 ± 0.082} & 0.032 ± 0.007 & 0.225 ± 0.057 & 0.838 ± 0.006 \\
\rowcolor{Wheat1} DecisionTree Platt & 0.106 ± 0.007 & 0.529 ± 0.064 & 0.059 ± 0.003 & 0.261 ± 0.03 & 0.836 ± 0.006 \\
\rowcolor{Wheat1} DecisionTree Temp & 0.098 ± 0.003 & 0.3 ± 0.026 & 0.091 ± 0.002 & 0.232 ± 0.016 & 0.841 ± 0.005 \\
\rowcolor{Wheat1} DecisionTree Isotonic & 0.055 ± 0.024 & 0.292 ± 0.039 & 0.042 ± 0.017 & 0.235 ± 0.046 & 0.836 ± 0.006 \\
\midrule
NaiveBayes ERM & 0.277 ± 0.019 & 0.469 ± 0.031 & 0.164 ± 0.013 & 0.266 ± 0.025 & 0.714 ± 0.018 \\
NaiveBayes $\hkrr$ & 0.019 ± 0.002 & 0.311 ± 0.08 & \highest{0.018 ± 0.002} & 0.217 ± 0.043 & \highest{0.84 ± 0.002} \\
NaiveBayes $\hjz$ & 0.027 ± 0.005 & 0.311 ± 0.037 & 0.026 ± 0.002 & 0.284 ± 0.027 & 0.826 ± 0.0 \\
NaiveBayes Platt & 0.268 ± 0.008 & 0.452 ± 0.012 & 0.164 ± 0.005 & 0.268 ± 0.01 & 0.719 ± 0.007 \\
NaiveBayes Temp & 0.298 ± 0.003 & 0.343 ± 0.006 & 0.276 ± 0.002 & 0.307 ± 0.004 & 0.719 ± 0.007 \\
NaiveBayes Isotonic & \highest{0.017 ± 0.002} & \highest{0.216 ± 0.06} & 0.019 ± 0.001 & \highest{0.205 ± 0.055} & 0.829 ± 0.006 \\
\bottomrule
\end{tabular}


==> tables/data_reuse/MEPS_table_short.tex <==
\begin{tabular}{llllll}
\toprule
\textbf{{Model}} & \textbf{{ECE}} $\downarrow$ & \textbf{{Max ECE}} $\downarrow$ & \textbf{{smECE}} $\downarrow$ & \textbf{{Max smECE}} $\downarrow$ & \textbf{{Acc}} $\uparrow$ \\
\midrule
\rowcolor{Wheat1} MLP ERM & 0.024 ± 0.006 & 0.107 ± 0.018 & 0.026 ± 0.004 & 0.1 ± 0.025 & \highest{0.865 ± 0.002} \\
\rowcolor{Wheat1} MLP $\hkrr$ & 0.024 ± 0.006 & 0.109 ± 0.022 & 0.024 ± 0.006 & 0.096 ± 0.016 & 0.862 ± 0.003 \\
\rowcolor{Wheat1} MLP $\hjz$ & 0.018 ± 0.001 & 0.105 ± 0.011 & 0.021 ± 0.002 & 0.093 ± 0.021 & 0.864 ± 0.003 \\
\rowcolor{Wheat1} MLP Isotonic & \highest{0.017 ± 0.004} & \highest{0.081 ± 0.008} & \highest{0.019 ± 0.002} & \highest{0.07 ± 0.009} & 0.863 ± 0.002 \\
\midrule
RandomForest ERM & \highest{0.017 ± 0.001} & 0.091 ± 0.005 & \highest{0.02 ± 0.001} & 0.082 ± 0.005 & 0.862 ± 0.002 \\
RandomForest $\hkrr$ & 0.089 ± 0.004 & 0.25 ± 0.026 & 0.088 ± 0.004 & 0.221 ± 0.025 & 0.848 ± 0.002 \\
RandomForest $\hjz$ & 0.022 ± 0.003 & \highest{0.088 ± 0.007} & 0.024 ± 0.001 & 0.083 ± 0.004 & 0.862 ± 0.002 \\
RandomForest Isotonic & 0.075 ± 0.002 & 0.167 ± 0.005 & 0.058 ± 0.002 & 0.121 ± 0.007 & 0.86 ± 0.003 \\
\midrule
\rowcolor{Wheat1} SVM ERM & 0.149 ± 0.015 & 0.359 ± 0.04 & 0.075 ± 0.008 & 0.179 ± 0.019 & 0.851 ± 0.015 \\
\rowcolor{Wheat1} SVM $\hkrr$ & 0.018 ± 0.005 & \highest{0.111 ± 0.013} & 0.018 ± 0.005 & \highest{0.101 ± 0.006} & 0.853 ± 0.01 \\
\rowcolor{Wheat1} SVM $\hjz$ & 0.06 ± 0.007 & 0.211 ± 0.069 & 0.048 ± 0.009 & 0.183 ± 0.055 & \highest{0.857 ± 0.006} \\
\rowcolor{Wheat1} SVM Isotonic & \highest{0.007 ± 0.004} & 0.202 ± 0.057 & \highest{0.007 ± 0.004} & 0.195 ± 0.051 & 0.852 ± 0.014 \\
\midrule
LogisticRegression ERM & 0.022 ± 0.002 & 0.106 ± 0.008 & 0.022 ± 0.001 & 0.083 ± 0.003 & \highest{0.866 ± 0.002} \\
LogisticRegression $\hkrr$ & 0.024 ± 0.001 & 0.12 ± 0.011 & 0.023 ± 0.001 & 0.105 ± 0.009 & 0.861 ± 0.003 \\
LogisticRegression $\hjz$ & 0.022 ± 0.003 & 0.106 ± 0.011 & 0.022 ± 0.002 & 0.083 ± 0.005 & 0.866 ± 0.001 \\
LogisticRegression Isotonic & \highest{0.014 ± 0.002} & \highest{0.087 ± 0.01} & \highest{0.018 ± 0.002} & \highest{0.073 ± 0.002} & 0.866 ± 0.001 \\
\midrule
\rowcolor{Wheat1} DecisionTree ERM & \highest{0.067 ± 0.006} & 0.266 ± 0.029 & \highest{0.048 ± 0.004} & 0.17 ± 0.013 & 0.849 ± 0.007 \\
\rowcolor{Wheat1} DecisionTree $\hkrr$ & 0.074 ± 0.007 & 0.282 ± 0.034 & 0.073 ± 0.007 & 0.237 ± 0.022 & 0.845 ± 0.007 \\
\rowcolor{Wheat1} DecisionTree $\hjz$ & 0.068 ± 0.007 & 0.264 ± 0.035 & 0.049 ± 0.005 & 0.167 ± 0.018 & \highest{0.849 ± 0.007} \\
\rowcolor{Wheat1} DecisionTree Isotonic & \highest{0.067 ± 0.006} & 0.266 ± 0.029 & \highest{0.048 ± 0.004} & 0.17 ± 0.013 & 0.849 ± 0.007 \\
\midrule
NaiveBayes ERM & 0.277 ± 0.019 & 0.544 ± 0.02 & 0.164 ± 0.013 & 0.287 ± 0.011 & 0.714 ± 0.018 \\
NaiveBayes $\hkrr$ & 0.023 ± 0.003 & \highest{0.119 ± 0.026} & 0.023 ± 0.003 & \highest{0.102 ± 0.019} & 0.833 ± 0.005 \\
NaiveBayes $\hjz$ & 0.05 ± 0.017 & 0.205 ± 0.038 & 0.044 ± 0.014 & 0.183 ± 0.038 & 0.803 ± 0.004 \\
NaiveBayes Isotonic & \highest{0.014 ± 0.002} & 0.121 ± 0.009 & \highest{0.017 ± 0.001} & 0.111 ± 0.005 & \highest{0.834 ± 0.006} \\
\bottomrule
\end{tabular}


==> tables/groups/YelpPolarity.tex <==
\begin{tabular}{lrll}
\toprule
group name & n samples & fraction & y mean \\
\midrule
pricey & 9333 & 0.0156 & 0.6610 \\
expensive & 21053 & 0.0352 & 0.4439 \\
cheap & 27383 & 0.0458 & 0.4509 \\
affordable & 4098 & 0.0069 & 0.8346 \\
overpriced & 10764 & 0.0180 & 0.1564 \\
service & 159446 & 0.2666 & 0.4340 \\
ambiance & 9418 & 0.0157 & 0.6448 \\
time & 203289 & 0.3399 & 0.4672 \\
location & 44839 & 0.0750 & 0.4603 \\
late & 87913 & 0.1470 & 0.4310 \\
early & 29048 & 0.0486 & 0.3888 \\
loud & 12824 & 0.0214 & 0.3670 \\
breakfast & 22701 & 0.0380 & 0.5857 \\
lunch & 40771 & 0.0682 & 0.5793 \\
dinner & 41944 & 0.0701 & 0.5362 \\
sandwich & 28563 & 0.0478 & 0.5522 \\
pizza & 27493 & 0.0460 & 0.5355 \\
salad & 38790 & 0.0649 & 0.5495 \\
fish & 21431 & 0.0358 & 0.5091 \\
grill & 13159 & 0.0220 & 0.5647 \\
pasta & 9873 & 0.0165 & 0.5129 \\
burger & 28573 & 0.0478 & 0.5204 \\
sushi & 17450 & 0.0292 & 0.5310 \\
drinks & 41409 & 0.0692 & 0.4554 \\
coffee & 20491 & 0.0343 & 0.5657 \\
salty & 8736 & 0.0146 & 0.3500 \\
sweet & 29773 & 0.0498 & 0.6476 \\
large & 30807 & 0.0515 & 0.5705 \\
small & 50182 & 0.0839 & 0.4865 \\
hype & 4710 & 0.0079 & 0.2705 \\
terrible & 16585 & 0.0277 & 0.0716 \\
incredible & 5199 & 0.0087 & 0.8517 \\
love & 84159 & 0.1407 & 0.7220 \\
again & 80913 & 0.1353 & 0.3510 \\
\midrule
Dataset & 598000 & 1.0000 & 0.5000 \\
\bottomrule
\end{tabular}

